OmniPhys: Knowledge-Graph-Driven Benchmarking and Collective Optimization for Physical Commonsense in Text-to-Image Generation

While text-to-image models exhibit remarkable visual fidelity, they frequently violate fundamental physical commonsense. Existing benchmarks often rely on coarse-grained descriptions, failing to diagnose the mastery of specific physical principles. Moreover, the high stochasticity of generative processes causes current prompt optimization methods to suffer from gradient hallucinations, where optimizers are misled by transient visual artifacts rather than systemic flaws. To address these challenges, we introduce OmniPhys, a rigorous benchmark of 1,551 samples grounded in a Physical Knowledge Graph. By aligning PhET simulations with standard curricula, OmniPhys operationalizes a knowledge-to-scenario pipeline that performs diagnostic stress tests via a dual-path verification protocol. We further propose OmniPrompt, an iterative framework that treats physical alignment as a discrete optimization problem. For each query, OmniPrompt aggregates K stochastic images into a per-query feedback buffer. Across training, it further merges feedback from batches of B queries before each meta-policy update, filtering seed and query-local noise. Evaluations across 12 representative text-to-image models reveal universal physical bottlenecks. Results demonstrate that OmniPrompt significantly enhances physical consistency across diverse backbones, proving the transferability and efficacy of our evolved meta-policies. The code and data are available at https://github.com/zjukg/OmniPhys

==> new_results.tex <==
\begin{table*}[htbp] % 使用 table* 环境可跨双栏（适用于双栏模板）；单栏模板用 table 即可
\centering
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & 
\multirow{2}{*}{\textbf{Strategy}} & 
\multicolumn{3}{c}{\textbf{Machines}} & 
\multicolumn{3}{c}{\textbf{Optics}} & 
\multicolumn{3}{c}{\textbf{Object}} & 
\multicolumn{3}{c}{\textbf{overall}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(l){12-14}
& & VQA & DCS & Joint & VQA & DCS & Joint & VQA & DCS & Joint & VQA & DCS & Joint \\
\midrule
FLUX 1.0 & None (raw query) &  &  &  &  &  &  &  &  &  & 0.389 & 0.132 & 0.110  \\
         & Two-Stage Reasoning &  &  &  &  &  &  &  &  &  & 0.478 & 0.252 & 0.205  \\
         & Instance-level Optimization &  &  &  &  &  &  &  &  &  & 0.465 & 0.260 & 0.209  \\
         & Collective Optimization (our) &  &  &  &  &  &  &  &  &  & 0.478 & 0.281 & 0.221 \\
\midrule
JanusPro-7B & None (raw query) &  &  &  &  &  &  &  &  & & 0.333 & 0.100 & 0.071 \\
            & Two-Stage Reasoning &  &  &  &  &  &  &  &  & & 0.499 & 0.305 & 0.230  \\
            & Instance-level Optimization &  &  &  &  &  &  &  &  &  & 0.522& 0.321 & 0.244  \\
            & Collective Optimization (our) &  &  &  &  &  &  &  &  &  & 0.523 & 0.322 & 0.254  \\
\midrule
Lumina-Image & None (raw query) &  &  &  &  &  &  &  &  &  & 0.365 & 0.126 & 0.102 \\
             & Two-Stage Reasoning &  &  &  &  &  &  &  &  &  & 0.465 & 0.243 & 0.200  \\
             & Instance-level Optimization &  &  &  &  &  &  &  &  & &0.469 &0.234 & 0.189  \\
             & Collective Optimization (our) &  &  &  &  &  &  &  &  & & 0.472 & 0.266 & 0.214 \\
\bottomrule
\end{tabular*}
\caption{Performance comparison across physical scenarios (Machines, Optics, Object) and overall metrics.}
\label{tab:performance}
\end{table*}
